Unveiling Diversity: Empowering OSS Project Leaders with Community Diversity and Turnover Dashboards

Managing open-source software (OSS) projects requires managing communities of contributors. In particular, it is essential for project leaders to understand their community's diversity and turnover. We present CommunityTapestry, a dynamic real-time community dashboard, which presents key diversity and turnover signals that we identified from the literature and through participatory design sessions with stakeholders. We evaluated CommunityTapestry with an OSS project's contributors and Project Management Committee members, who explored the dashboard using their own project data. Our study results demonstrate that CommunityTapestry increased participants' awareness of their community composition and the diversity and turnover rates in the project. It helped them identify areas of improvement and gave them actionable information.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> Sections/1._Intro.tex <==
\section{Introduction}
\label{sec:intro}
Diversity has been shown to have many positive effects on organizations, including a better ability to innovate, a better reputation as ethical citizens, and a better ``bottom line'' for businesses ~\cite{phillips2014diversity, page2019diversity, larkin2020diversity}. 

Research has investigated the influence of different diversity factors on productivity in Open Source Software (OSS). 
For instance, studies have demonstrated the impact of gender diversity on productivity~\cite{vasilescu2015gender} and the significance of organization affiliation diversity in ensuring project sustainability and success~\cite{yin2021sustainability}. Research also suggests that the concept of \emph{coopetition}, where competing companies use OSS to collaborate on shared challenges, leads to reduced workload, heightened productivity, and improved product quality~\cite{guizani2023rules}. 
On the other hand, a non-diverse community signals an unwelcoming environment to companies signifying a lack of neutral governance \cite{guizani2021long}, or to individuals signifying an non-inclusive environment \cite{guizani2022perceptions}. This can, in turn, result in a high turnover rate \cite{sharma2012examining, foucault2015impact}, where OSS projects struggle to attract and retain diverse contributors, especially women~\cite{terrell2017gender, lee2019floss}. 

Some project leaders recognize the positive effects of diversity, the adverse effects of lack thereof, and desire more diversity in their projects~\cite{qiu2023climate}. However, they struggle to find the time and bandwidth to monitor the state of diversity in their community and may miss important signals as explained by a Lead Program Manager for a Large OSS Company~\cite{germonprez2018eight}: \textit{``We try to determine the rough diversity of employment in our projects. The rough metric we have is about two-thirds of our contributors do not work for our primary corporate sponsor. That is extraordinarily critical when you look at both the objectives of our primary sponsor as well as the health of the community.''} 

In fact, keeping on top of everyday project tasks, such as pull-request reviews to ensure software quality, is already a challenge for project leaders~\cite{ferreira2021shut}. Project leaders report being stressed and feeling burnout, overwhelmed by the number of requests they receive (e.g., bug reports, support requests)~\cite{raman2020stress}. Hence, a more systematic support of monitoring diversity and implementing actions to improve it is necessary.

%\todo{Unfortunately, so far lion's share of research has focused on understanding diversity and inclusion in OSS and contributors' experiences \cite{guizani2021long, rodriguez-perez2021slr, steinmacher2013newcomers, steinmacher2015social, trinkenreich2020hidden, feng2023state, trinkenreich2021pots}}\as{ rather than on providing the aforementioned systematic monitoring support. }

Thus far, research has largely focused on getting a deep understanding of different aspects of diversity and inclusion in OSS and contributors' experiences \cite{guizani2021long, rodriguez-perez2021slr, steinmacher2013newcomers, steinmacher2015social, trinkenreich2020hidden, feng2023state, trinkenreich2021pots}. 
It is now time to provide the aforementioned systematic monitoring support.
%
%\todo{
So far monitoring has been limited to research-driven dashboards focusing on the health of OSS teams and project sustainability~\cite{qiu2023climate,guizani2022attracting, ramchandran2022exploring}. 
%For instance, \citet{qiu2023climate} and \citet{guizani2022attracting} developed dashboards to aid maintainers in understanding their communities and attracting newcomers, highlighting project goals, and recognizing contributors' efforts. 
These dashboards, however, do not look at diversity specifically. Not having such a lens can hide problem spots (such as women leaving the project) within the larger trends of overall contributors. 
%Despite these efforts, when looking at interventions that focus specifically on diversity lenses, there remains a gap between the vast body of empirical knowledge on diversity and inclusion and the practical implementation of actionable solutions. }
%\todo{Here we create a dashboard that makes the diversity lenses a first order entity...allowing people to look at trends and data disaggregated for a specific lens, that can bring out stuff that would be hidden otherwise}
In this paper, we close this gap and complement the current body of interventions by designing and deploying a systematic monitoring support focused on turnover, gender and affiliation diversity.



% For instance, \citet{qiu2023climate} created a dashboard to help maintainers understand their community composition and activity including the conversation tone and  \citet{guizani2022attracting} designing a dashboard to maintainers attract and retain newcomers by highlighting project goals (e.g., a social good cause) and recognizing active newcomers (e.g., a ``rising contributor'' badge).


%\as{I am not sure that we need this: ``To the best of our knowledge, the only interventions that address diversity lenses are ones in the GenderMag method space \cite{burnett2016gendermag, guizani2022debug,chatterjee2021aid}. The GenderMag method has a cognitive walkthrough method that helps enhance the inclusivity of the tools themselves (e.g., OSS project) to reduce the cognitive burden on users with diverse cognitive learning styles \cite{burnett2016gendermag}. One such intervention is the Why/Where/Fix process that uses GenderMag and Information Architecture to systematically find and fix inclusivity bugs within the tool itself (e.g., OSS project) \cite{guizani2022debug}. We used this method to remove inclusivity bugs from CommunityTapestry.''}
%}

%Two notable exception of diversity lenses: 
%Dashboard intervention 
%Process intervention 
%community intervention 
%focus monitoring the community 


We developed a dynamic real-time dashboard named CommunityTapestry through participatory design (PD) \cite{schuler1993participatory}. The goal of CommunityTapestry is to: (1) signal to project leaders the specific state of their project diversity and turnover rate, (2) give them information to take actions relevant to their project needs and (3) help monitor the effects of their actions over time.


We used a large Apache Source Foundation (ASF) project, Project~B\footnote{As per our agreement with Project~B, we use pseudonyms to avoid any negative impressions about the project, as well as to protect the identity of individuals.} in our PD study. 
PD allowed us to work closely with the project community stakeholders to better understand their needs, constraints, and priorities. An additional benefit is that having the stakeholders as partners engendered an interest and investment in the project, which in turn improved the chances of the dashboard being adopted by the community. The stakeholders were the Project Management Committee (PMC) chair of Project~B, Project~B community manager, the Diversity and Inclusion vice-president of the ASF, and an engineer working on GrimoireLab \cite{duenas2021grimoirelab}, our dashboard infrastructure. We refer to them from now on as our PD partners.


Through discussions with our PD partners, we prioritized the diversity lenses (gender and organization affiliation) and the project-related activities (e.g., trends of newcomers joining or contributors leaving, communication network) of interest. We then used PD principles~\cite{schuler1993participatory} of collaborative prototyping to design the dashboard, which we implemented and deployed on existing OSS infrastructure that the project uses, and evaluated it with future users. The study spanned 14 months, during which, we created CommunityTapestry and evaluated it for inclusivity (using the \textsc{Why/Where/Fix} approach, Section \ref{sec:evaluation1}) and its usefulness %with future users
(15 participants, Section \ref{sec:evaluation2}). 

Our results show that CommunityTapestry enabled participants to gain insight and awareness into their project diversity and turnover rate, and provided ammunition to take action.   


% \boldification{the contributions of this paper are...}
% The contributions of this paper is a deployed Dynamic Real-time Dashboard named CommunityTapestry that helps (1) signal to project leaders the specific state of their project diversity and turnover rate, (2) give them information to take actions relevant to their project needs and (3) can help monitor their effect over time. %\as{Did we ask the interviewees whether they felt empowered? If not, how can we prove (2)?} \mg {we asked participants: whether the dashboard helped identify aspects to improve and whether the dashboard will have an effect on their actions. @Alexander, should we change the word empower to identify improvements? } \as{Maybe yes. @Anita, what do you think?} \mg{Anita says, yes don't use empower, let's say "give them information to"}

% \boldification{We leveraged participatory design with stakeholders to identify key factors to track }
% For this tool to be used by the community, we wanted to understand the community needs. To this end, we leveraged participatory design~\cite{preece1994human} with stakeholders to identify key factors and measures 
% %\as{What is the difference between ``factors'' and ``measures''?} \mg{I understand factor as a component (e.g., gender, types of contribution) and measure as a way to quantify a factor} 
% indicative of community diversity and turnover that are not currently addressed in existing infrastructures, such as indicators of gender and affiliation diversity in project activities, communication, turnover, and trends of attraction and retention. 
% %
%  We continued to involve our stakeholders throughout the design and implementation processes sharing and reflecting on multiple designs and artifacts (e.g., requirements, low fidelity, and high fidelity prototypes). 
% %\as{What are these artifacts?} \mg{added examples}
% We evaluated our dashboard with 15 project leaders 
% %(i.e, Project Management Committee Members (PMC), committers)
% of a large Apache Software Project that we will call Project~B. 
% %\as{Why is the project anonymous? In any case, please use a macro here.} \mg{Anita suggested keeping it anonymous}
% %
% Prior to the user study, we tested the dashboard for inclusivity bugs using a systematic  debugging process~\cite{guizani2022debug}, sandboxed, and piloted our study. 
% \boldification{the contribution of this work is the building, deployment, and evaluation of CommunityTapestry a Dynamic Real-time Dashboard (RDD) that can help increase awareness, inspire action, and monitors their effect over time}

% Our results show that CommunityTapestry enabled project leaders to gain insight and awareness into their project diversity and turnover rate, and provided ammunition to take action.   



%The significance of diversity and its effect on organizations has been widely acknowledged. \as{\cn}
% What many organizations hope to gain from diverse teams is diversity of information and of thought \cite{phillips2014diversity}. 

%Information processing theory \cite{salancik1978social} shows the positive effects of diversity by bringing to light that access to different networks and broader information can enhance a team’s creativity, adaptability, and problem solving skills \cite{jackson2004diversity, watson1993cultural}

%These findings offer insights into the composition of OSS projects, with company-based projects constituting the majority (59.9\%) within the Apache Software Foundation (ASF). The drive to foster community development and diversity emerges as a key motivation for project participation \cite{yang2022projects}, aligning with the objective of promoting neutral governance \cite{guizani2023rules}.
%When diversity is not supported, the overall health and sustainability of OSS project is in question. 
%\as{What do we mean by not supporting diversity?}

%when they lack, \as{When factors lack or when diversity is lacking? Please rephrase} 

%\as{Do we have any evidence that they actually struggle? Quotes? Bibliographic references?}
%\as{Would the following quote form Germonprez et al.~\cite{germonprez2018eight} be sufficient to support our claim? “We try to determine the rough diversity of employment in our projects. The rough metric we have is about two-thirds of our contributors do not work for our primary corporate sponsor. That is extraordinarily critical when you look at both the objectives of our primary sponsor as well as the health of the community too.”— Lead Program Manager for a Large Open Source Software Company}
%\mg{thank you, added the quote above}
%\as{Are leaders and managers the same? If yes, let us use one of the terms.} \mg{yes, done} % Social coding platforms (e.g., GitHub) have incorporated metrics to capture OSS contributions (e.g., commit frequency) and signal the presence of standards (e.g., readme, code of conduct).  %\as{I agree. However, it is not the case that there are no interventions at all. GenderMag, obviously, is one of such interventions.} \mg{changed to reflect that please, see edits above}


% boldifcation: 


% \boldification{Diversity has important positive effects on organization from innovation to reputation and a better bottom line }
% %
% \boldification{OSS is no stranger to the effect of diversity on productivity, sustainability, and success.... for example, gender diversity has this effect and affiliation diversity has that effect...}
% %
% \boldification{Despite the known positive and adverse effects of diversity, project leaders are often busy keeping the code base afloat and tend to miss signals...}
% %
% \boldification{previous research has made progress in empirically understanding the state of diversity and inclusion in OSS, but there is a need to translate this knowledge into practice and develop tools that signal the diversity and turnover state, inspire action, and monitor its effect...}
% %

%including social and technical networks, over time. By tracking ASF project downturn events, identifying longer-term engagements between developers, and enabling within-ASF project comparisons, this tool could potentially improve the likelihood of project graduation into ASF.}

%\textbf{qiu2023climate}: Dashboard that monitors the health of team management (e.g., Number of new contributors, active contributors), social capital (\# of new contributors, average experience of contributors), the responsiveness and conversation tone -- while focus specifically on diversity and turnover in our disaggregated data 



%improve contributors' experience and increase diversity and inclusion in OSS. One notable approach consisted of enhancing the inclusivity of the tools themselves (e.g., OSS project) to reduce the cognitive burden on users with diverse cognitive learning styles \cite{burnett2016gendermag, guizani2022debug,chatterjee2021aid}. Other research focused on improving newcomers' experience by creating a portal to support newcomers' onboarding in OSS \cite{steinmacher2016overcoming} and 
 %designing a dashboard to help attract and retain newcomers \cite{guizani2022attracting}. 
% To monitor the health of OSS teams and project sustainability \citet{qiu2023climate} created a dashboard that incorporates signals of team management, social capital, and conversation tone and \citet{ramchandran2022exploring} devised a dashboard to track the sustainability trajectories of nascent projects within the Apache Software Foundation, identifying downturn events and fostering longer-term developer engagements.

==> Sections/3._DesignImplementation.tex <==
\section{Research Method}
\label{sec:design}

Our work is a PD study, where designers work closely with users to establish requirements and investigate how to combine existing technologies and structures with future technologies \cite{bodker2022participatory}. We adopted the following PD practices: (1) \textit{collaborative prototyping,} 
where non-designers can express ideas through accessible design materials and future users can gain hands-on experience with the future technology, (2) \textit{infrastructuring}, where designers and users establish organizational and technical infrastructures to ensure results of the project can be sustained after the project ends, and (3) \textit{evaluation}, where future users assess the qualities
of a design product and the outcomes emerging from the design process.


We worked with the Apache Software Foundation (ASF) and one of their projects (Project~B), a large Big-Data-related project comprising more than 1000 current contributors. The Project Management Committee (PMC) chair of Project~B, a community manager of Project~B, the Diversity and Inclusion vice-president of the ASF, and an engineer working on GrimoireLab \cite{duenas2021grimoirelab}, upon which we implement the dashboard, were our partners in the PD study (We refer to them here on as our PD partners). Through this project, we designed, infrastructured, and evaluated the CommunityTapestry over a \textit{period of 14 months}.


\subsection{Collaborative Prototyping}
\label{designsubsection}


Prototyping in Participatory Design is collaborative, where non-designers can express ideas through accessible design materials. We started the design phase by first discussing: (1) the different aspects of diversity---gender, affiliation, race, and age, and (2) the data to use in the dashboard (outcome variables)---Number of contributors left/ might be leaving, Time to merge PR. 


We started by discussing the survey responses of a contributor survey that the ASF had recently completed ($N>400$), which included contributors' demographics and the challenges they faced disaggregated by demographics. We then prioritized the diversity lenses of interest to Project~B and the ASF, which could be implemented from data that GrimoireLab collects. For instance, we discussed but did not include race, an important diversity lens. Inferring race from GitHub profiles is not feasible; the definition of race is not consistent across countries and is a deeply sensitive aspect, which, if surfaced, can have a negative impact on the individual. \textit{Organization affiliation} and \textit{Gender} were selected as our lenses. 


Next, we prioritized the outcome variables that were relevant to our PD partners (see Section \ref{sec:walkthrough}). For instance, we dropped the leadership outcome variables as project leadership teams tend to be small groups of people who already know each other. 

We then created interactive mockups of the dashboards using Figma\footnote{\url{https://www.figma.com/prototyping/}}. We met bi-weekly with our PD partners to refine our prototypes. During these (online) meetings, our PD partners performed walkthroughs of the dashboard while thinking aloud and sharing their screens. They provided feedback verbally or annotated on the screen share. All meetings were recorded (screen and audio).

The feedback ranged from changes or enhancement of existing features to requesting new features.  
For instance, we adjusted the network visualizations. The PR communication network, depicting communication among contributors during PR reviews (see Figure \ref{fig:dashboards-b}), was updated so that the thickness of edges between the contributor (nodes) reflected the number of PRs instead of the number of comments.
We also updated the PR communication network with a table displaying the PR details (e.g., URL, date of creation) that have not received any comments (nodes that isolate in the network visualization). 
After six meetings, the prototype features matched our PD partners' needs and constraints.


\subsection{Infrastructuring}
\label{infra}


A core concern in PD is to ensure that the participating organization is in a position where experiences can be used beyond the project. We, therefore, implemented CommunityTapestry as real-time dashboards in GrimoireLab \cite{duenas2021grimoirelab}, which is an open-source analytics toolkit and a part of the CHAOSS project \cite{duenas2021grimoirelab}.
GrimoireLab allowed us to integrate real-time data across multiple platforms such as GitHub repositories and Stack Overflow (see Figure \ref{fig:DashboardArchitecture}).  


\begin{figure}[!tbp]
\centering
\includegraphics[width=3 in]{figure/dashboardArchitecture.png}
\caption{Dashboard architecture using GrimoireLab \cite{duenas2021grimoirelab}.}
\label{fig:DashboardArchitecture}
\end{figure}


\textbf{Data Mining.} In accordance with the design agreed upon with our PD partners, we used GitHub, Git, and Stack Overflow as the primary data sources for CommunityTapestry (see Figure \ref{fig:DashboardArchitecture}). GrimoireLab leverages a Python API for fetching data from repositories, which enables us to access all retrieved items from the repositories as dictionaries (JSON documents), including PRs and PR comments. The Perceval library \cite{perceval} then streamlines the process of obtaining 24 hours of continuous updates from the repository, capturing only incremental changes. This not only ensures that our dashboard stays consistently current but it also provides immediate insight into the project's ongoing activities, thereby enabling project maintainers to take proactive measures in a timely manner.


\textbf{Meta-data and identity management.} Our dashboard uses SortingHat, a relational database-powered tool, to identify the activities of human contributors in an OSS project. Bots have become increasingly prevalent in contemporary software development for tasks such as automated code review \cite{wessel2021investigating, wessel2022effects}, and SortingHat allows us to filter out bot activities. 


SortingHat also helps us associate human contributors with their affiliations. For example, if a contributor's accounts in platforms such as GitHub, Git, and Stack Overflow are registered with a non-corporate domain like gmail.com, we classify their affiliation as ``affiliation unknown". However, if any of their accounts are associated with corporate domains such as google.com or apple.com, we can appropriately assign their contributions to the respective companies. This prioritization was a modification requested by our PD partners. Additionally, user IDs that are common across platforms are merged into a single entity (e.g, user@gmail and user@google.com are merged). 


The data retrieved from multiple sources is then analyzed and stored in Elasticsearch NoSQL database indexes \cite{elasticsearch}. 
GrimoireELK, another component of GrimoireLab, creates enriched indexes, an abstraction customized for our visualizations, and incorporates the merged identities generated by SortingHat. The enriched indexes then feed into the Kibiter/Kibana component \cite{kibana} to generate the visualizations for the dashboard. 


\textbf{Gender classification.} To infer the gender of contributors in our dataset, we used the Namsor API \cite{sebo2021performance}, a name recognition tool that estimates the gender of a full name on a -1 to +1 probability scale based on geographic information. During our initial iteration of gender classification, it became evident that relying solely on the location reported in a GitHub profile for predicting gender can lead to decreased precision. This is particularly true when the contributors' reported GitHub location does not align with the geographic origin of their name. For instance, this method posed significant difficulties when dealing with names from Asian countries such as China, Korea, and Japan. The process of transliterating names from pictographic characters to Latin letters can often lead to inaccuracies or multiple valid representations, as discussed by~\cite{kirnosova2021chinese}. As noted by Qiu et al.~\cite{Qiu.ea.2019}, this can cause the accuracy of gender prediction to drop significantly, in some cases falling below 30\%. 


To mitigate this issue, we implemented a two-step process. First, we used the Namsor API to predict the origin of contributors’ names. Then, we used both the predicted origin and their full names to predict their gender. To minimize prediction errors, we applied a threshold and filtered out gender predictions with probabilities lower than 90\%  in accordance with prior literature \cite{carsenat2019inferring, sebo2021performance}.


Next, we manually enhanced the precision of gender prediction. This task was undertaken by two researchers on our team: one of Chinese origin and the other an American of Japanese descent. Together, they identified the Asian names within our dataset and then equally divided the task of manual verification.
The manual verification process entailed cross-referencing the contributors' GitHub profiles and LinkedIn pages. If a profile page contained a clear photo or a stated pronoun, we used that information. In instances where the photo was unclear, the gender was marked as unknown. It is important to note that we acknowledge gender identity extends beyond a binary classification. As such, we have designed our system to be flexible, allowing for future updates and modifications to the database.


In total, we manually validated 991 names, out of which 559 remained unpredictable, as they did not provide any profile photo on their GitHub or LinkedIn page. 191 underwent double-validation and 45 required corrections from Namsor prediction results (3 from male to female and 42 from female to male). 


\section{Community Tapestry}
\label{sec:walkthrough}


Let us consider a hypothetical scenario in which Riley, a new PMC chair in Project~B, believes it important to be aware of and improve gender and affiliation diversity within their project. Figure~\ref{fig:walk} presents one of the dashboard pages of CommunityTapestry (see Figure \ref{fig:dashboards} for examples of other dashboards pages). The letters in the figure (e.g.,\protect\overviewLabelBig{C}.) identify the information we will explain below.


\begin{figure*}[!h]
    \centering    \includegraphics[width=0.6\linewidth]{figure/WTDash.png}
    \caption{Walkthrough of the CommunityTapestry contributor retention trend. Contributors' names and affiliations have been deducted for anonymization purposes.``A'' stands for affiliation and ``WC'' stands for woman contributor and ``MC'' is man contributor.}
    \label{fig:walk}
\end{figure*}


\begin{figure*}[!h]
    \centering
    \subfloat[\centering Types of contributions by affiliation dashboard]{{\includegraphics[width=5cm]{figure/Types.png} } \label{fig:dashboards-a}}%
    \qquad
    \subfloat[\centering Communication by gender dashboard]{{\includegraphics[width=9cm]{figure/Communication.png} } \label{fig:dashboards-b}}%
    \caption{Example of two of the dashboards of CommunityTapestry. Contributors' names and affiliations have been deducted for anonymization purposes. See Figure \ref{fig:walk} caption.}%
    \label{fig:dashboards}%
\end{figure*}


Riley begins by navigating to the dashboard ``Contribution Retention Trends'' in CommunityTapestry \protect\overviewLabelBig{A}. She notices the visualization that shows the trends of newcomers, contributors who left (i.e., inactive in the last six months), and might be 
leaving (i.e., inactive in the last 3 months), as well as the retention trend disaggregated by gender.
\protect\overviewLabelBig{B}. 
Using this information, Riley notices that while there is similar retention between men and women in the project (black line under contributor retention trends in \protect\overviewLabelBig{B}), there is a difference of 20/5 between men and women trends.


Riley decides to dive deeper. She filters the data to the last year. She reviews the detailed list of women contributors who might be leaving (the list contains name, \# contributions, affiliation, and last contribution date) to reach out to them, understands what is happening, and help if possible \protect\overviewLabelBig{C}. 


Note, CommunityTapestry allows filtering the visualizations by different criteria: time \protect\overviewLabelBig{D}, affiliation name and gender\protect\overviewLabelBig{E}. These filters can be applied by clicking on the visualization or typing.


Riley wonders if the inactive women are because they were affiliated with a company that stopped contributing. She then looks at the list of contributors who might be leaving  \protect\overviewLabelBig{C}. 
Riley notices two women from the company ``A3''\footnote{We have anonymized the names and affiliations here for confidentiality reasons.} leaving the project, so she reaches out to them to find out if the reason was a personal decision or a company-related decision.


%Seeing this gender imbalance in the project, Riley decides to be proactive and look at newcomer women. 
%Riley scrolls down to the newcomers' visualization \protect\overviewLabelBig{F} and sees three women joining the project from different affiliations. Riley sends a welcoming email, offering help and mentorship, and checking to see if they have any open issues and PRs that need attention. 


\subsection{Additional dashboards \label{sec:dashboard}}


CommunityTrapestry has two additional dashboards that can be disaggregated by gender or affiliation. Each dashboard contains different visualizations that are described below.


\textit{\textbf{Communication.}} The communication dashboard (Figure~\ref{fig:dashboards-a}) depicts the PRs interactions between contributors, disaggregated by affiliation or gender. This dashboard has four visualizations. \textit{(1) PRs overview}, which shows the number of PRs by group (i.e., gender, affiliation), comments, and likes. \textit{(2) Time to merge PRs}, displays the average time (in days) a group (i.e., gender, affiliation) has to wait to get their PR merged in descending order. \textit{(3) PRs communication network} is a graph where nodes are contributors, and the edges link contributors commenting and reviewing on the same PR. The size of the nodes reflects the number of PRs authored by a contributor, and the thickness of an edge reflects the number of PRs between two nodes (i.e., contributors). The colors differentiate the disaggregated groups (i.e., gender, affiliation) and are displayed in a legend. \textit{(4) PRs that need attention}  lists PRs that did not receive any comments and their details. This visualization contains the links to the PRs and the contributor information (name, affiliation, gender).


\textit{\textbf{Types of Contributions}}. The types of contributions dashboard (Figure~\ref{fig:dashboards-b}) details the different kinds of contributions in an OSS project using the gender and affiliation lenses. This dashboard has four sets of visualizations. \textit{(1) Contributors}, this set contains two 
visualizations presenting the percentage of contributors and the total number of contributors, both broken down by affiliation or gender. \textit{(2) PRs}, this set has four visualizations: [i] PRs proportion over time which shows the percentage of PRs during a certain period of time disaggregated by gender or affiliation. [ii] PRs evolution over time displays the evolution of PRs counts over time by group (i.e., gender, affiliation). [iii] PRs count shows the total count of PRs within a group (i.e., gender, affiliation). [iv] PRs days to merge displays the number of days before merging a PR disaggregated by gender or affiliation. \textit{(3) Issues}, this set consists of four visualizations that are similar to the ones mentioned in \textit{(2)} but present information related to the issue's contributions. \textit{(4) StackOverflow}, this last set of four visualizations contains information on StackOverflow's questions and answers. This set is similar to information in \textit{(2)} and \textit{(3)}. All dashboard pages allow filtering by different criteria such as time, gender, and affiliation. 


==> tables/Stats.tex <==
\begin{table*}[htbp]
    \caption{Pre- and post-awareness and action statistic}
    \label{statsdist}
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \hline
        Question & Median & Mean & SD & t-test & sign-test & ES & Distributions\\
        \hline
        Q1: Gender diversity awareness & (4, 4) & (3.2, 4.4) & (1.16, 0.49) & skip & 0.25 & 0.64 & \includegraphics[width=2cm,height=1cm]{figure/distribution1.png}\\
        \hline
        Q2: Gender diversity action plan
        & (3.0 ,4.0) & (3.2 ,3.6) & (0.75, 1.02) & 0.18 & 0.25 & 0.39 & \includegraphics[width=2cm,height=1cm]{figure/distribution2.png}\\
        \hline
        Q3: Affiliation diversity awareness & (4.0 ,4.0) & (3.4, 4.2) & (0.8, 0.4) & skip & 0.25 & 0.52 & \includegraphics[width=2cm,height=1cm]{figure/distribution3.png}\\
        \hline
        Q4: Affiliation diversity action plan  & (3.0, 3.0) & (2.8, 3.2)  & (0.75, 0.74) & 0.18 & 0.25 & 0.48 & \includegraphics[width=2cm,height=1cm]{figure/distribution4.png}\\
        \hline
        Q5: Turnover awareness & (2.0, 4.0) & (2.4 ,4.0) & (1.01, 0) & *0.03 & 0.06 & 1.98 & \includegraphics[width=2cm,height=1cm]{figure/distribution5.png}\\
        \hline
        Q6: Turnover action plan & (2.0,3.0) & (2.2,3.0) & (0.39, 0.89) & skip & 0.12 & 0.48 & \includegraphics[width=2cm,height=1cm]{figure/distribution6.png} \\
        \hline
        
    \end{tabular}
\end{table*}



==> tables/outcome_variable.tex <==
\begin{table}[tbp]
\caption{Outcomer variables}
\centering
\resizebox{3.5in}{!}{
\begin{tabular}{llll}
\rowcolor[HTML]{EFEFEF} 
\textbf{D\&I lens} & \textbf{References} & \textbf{Outcome variables} & \textbf{References} \\
Gender & \cite{imtiaz2019investigating, terrell2017gender,Vasilescu-Bogdan-2015,vasilescu2012gender,wagner2015s} & Num\_contributors & \cite{eluri2021predicting,yamashita2016magnet,zhou2016inflow,guizani2022attracting} \\
\rowcolor[HTML]{EFEFEF} 
%Senority & \cite{Steinmacher.Wiese.ea_2012a,Musicant.Ren.ea_2011,Steinmacher.Silva.ea_2014,steinmacher2015systematic,steinmacher2013newcomers} & Num\_Pull Request (PR)/overtime & \cite{Ford.ea.2019, terrell2017gender,github_pull_requests,rahman2014insight,moreira2021factors} \\
Affiliation & \cite{guizani2023rules,yang2022projects,zhang2019companies} & Num\_PR comments/overtime & \cite{feng2022case, hu2012reputation,tsay2014influence} \\
\multicolumn{2}{l}{} & \cellcolor[HTML]{EFEFEF}Num\_Issues/overtime & \cellcolor[HTML]{EFEFEF}\cite{bissyande2013got,dhasade2020towards,panichella2021won} \\
\multicolumn{2}{l}{} & Num\_Stackoverflow Q\&A/overtime & \cite{barua2014developers, vasilescu2013stackoverflow} \\
\multicolumn{2}{l}{} & \cellcolor[HTML]{EFEFEF}Issue: days to first attention & \cellcolor[HTML]{EFEFEF}\cite{tan2020first,kikas2016using,zhou2020studying} \\
\multicolumn{2}{l}{} & PR: Time to merge & \cite{Terell-2017,terrell2017gender,chen2019replication,zhao2019improving} \\
\multicolumn{2}{l}{} & \cellcolor[HTML]{EFEFEF}PR: open without comments & \cellcolor[HTML]{EFEFEF}\cite{Terell-2017,terrell2017gender, hu2012reputation} \\
\multicolumn{2}{l}{} & Stackoverflow: average accepted answers & \cite{choetkiertikul2015will,zhang2019empirical,rahman2015insight} \\
\multicolumn{2}{l}{} & \cellcolor[HTML]{EFEFEF}PR comments: communication network & \cellcolor[HTML]{EFEFEF}\cite{feng2022case,singh2010small, hu2012reputation,tsay2014influence} \\
\multicolumn{2}{l}{} & Contributor retention/overtime & \cite{eluri2021predicting,yamashita2016magnet,zhou2016inflow,guizani2022attracting} \\
\multicolumn{2}{l}{\multirow{-9}{*}{}} & \cellcolor[HTML]{EFEFEF}Num\_contributor left/ might be leaving & \cellcolor[HTML]{EFEFEF}\cite{eluri2021predicting,yamashita2016magnet,zhou2016inflow,guizani2022attracting} \\
\multicolumn{2}{l}{\multirow{-9}{*}{}} & \cellcolor[HTML]{EFEFEF}Num\_new contributors & \cellcolor[HTML]{EFEFEF}\cite{steinmacher2013newcomers, steinmacher2015social}
\end{tabular}}
\label{tab:OV}
\end{table}

==> tables/suggestions.tex <==
% \usepackage{tabularray}
\begin{table}
\noindent\begin{tabularx}{\textwidth}{|l|l|X|X|X|}
\textbf{Lens} & \textbf{Feature} & \textbf{Where} & \textbf{About} & \textbf{Suggestion(s) from transcript}\\
Affiliation & Communication & Table & PR & Within affiliation vs between affiliations as an average for commenting\/average time for response  potential line graph Time to acknowledge\/responsiveness within affiliation vs between affiliations: goal is to be more responsive to people outside of affiliation so they feel more welcome\\
Gender & Types of Contributions & Trends & Newcomers (issues, PR) & Questions if spikes are due to existing contributors engaging more or new contributors that they didn't reach out to and left--the situation of the spikes SEEING NEW CONTRIBUTORS (a name that appears in commit history that didn't appear in previous history release) VS EXISTING CONTRIBUTORS\\
Gender & Types of Contributions &  & Newcomer attraction, activity, retention trend & Interest in gradual progression: when someone makes their second commit/comment, or third/fourth--like a retention line trend (this month how many out of the past month contributed, compare month t to the previous t - 1) THE EVOLUTION OF NEWCOMERS\\
Gender And Affiliation & Communication & Network & PR & Number of pull request comments isn't that interesting--more interesting how many people a node is connected to (not much the size of the node) + table\\
Gender & Communication & Network & PR & A single pull request with two people communicating back and forth counts as one\\
Gender & Communication & Network & PR & node size to represent pull requests instead of comments and edge number of mutual pull requests\\
Gender + affiliation & Table & Everywhere &  & Gender classification accuracy needs to be better\\
Gender & Types of Contributions &  & Spelling & Histogram is misspelled\\
Gender And Affiliation & Communication &  & PR & Table with people that are not connected to the network. people that we have not responded to\\
Affiliation & Types of Contributions &  & Affiliation classification & Someone with multiple affiliations - priorotize money first--affiliate with who is paying them (https://github.com/apache/beam/blob/master/.mailmap)
\end{tabularx}
\end{table}
